Learning NEAT Emergent Behaviors in Robot Swarms

When researching robot swarms, many studies observe complex group behavior emerging from the individual agents' simple local actions. However, the task of learning an individual policy to produce a desired group behavior remains a challenging problem. We present a method of training distributed robotic swarm algorithms to produce emergent behavior. Inspired by the biological evolution of emergent behavior in animals, we use an evolutionary algorithm to train a population of individual behaviors to produce a desired group behavior. We perform experiments using simulations of the Georgia Tech Miniature Autonomous Blimps (GT-MABs) aerial robotics platforms conducted in the CoppeliaSim simulator. Additionally, we test on simulations of Anki Vector robots to display our algorithm's effectiveness on various modes of actuation. We evaluate our algorithm on various tasks where a somewhat complex group behavior is required for success. These tasks include an Area Coverage task and a Wall Climb task. We compare behaviors evolved using our algorithm against designed policies, which we create in order to exhibit the emergent behaviors we desire.

==> misc/NEAT_table.tex <==
\begin{table}[htbp]
\caption{NEAT Parameter Selection}
\begin{center}
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Evolutionary Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}\\
\hline
pop\_size & 300\\
\hline
reset\_on\_extinction & False\\
\hline
no\_fitness\_termination & True\\
\hline
\multicolumn{2}{|c|}{\textbf{Stagnation Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}\\
\hline
species\_fitness\_func & mean\\
\hline
max\_stagnation & 20\\
\hline
species\_elitism & 2\\
\hline
\multicolumn{2}{|c|}{\textbf{Reproduction Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}\\
\hline
elitism & 2\\
\hline
survival\_threshold & 0.2\\
\hline
min\_species\_size & 2\\
\hline
\multicolumn{2}{|c|}{\textbf{Species Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}\\
\hline
compatibility\_threshold & 3.0\\
\hline
\multicolumn{2}{|c|}{\textbf{Genome Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}\\
\hline
activation\_default & sigmoid\\
\hline
activation\_mutate\_rate & 0.0\\
\hline
activation\_options & sigmoid\\
\hline
aggregation\_default & sum\\
\hline
aggregation\_mutate\_rate & 0.0\\
\hline
aggregation\_options & sum\\
\hline
bias\_init\_mean & 0.0\\
\hline
bias\_init\_stdev & 1.0\\
\hline
bias\_init\_type & gaussian\\
\hline
bias\_max\_value & 30.0\\
\hline
bias\_min\_value & -30.0\\
\hline
bias\_mutate\_power & 0.5\\
\hline
bias\_mutate\_rate & 0.7\\
\hline
bias\_replace\_rate & 0.1\\
\hline
compatibility\_disjoint\_coefficient & 1.0\\
\hline
compatibility\_weight\_coefficient & 0.5\\
\hline
conn\_add\_prob & 0.5\\
\hline
conn\_delete\_prob & 0.5\\
\hline
enabled\_default & True\\
\hline
enabled\_mutate\_rate & 0.01\\
\hline
feed\_forward & True\\
\hline
initial\_connection & full\_nodirect\\
\hline
node\_add\_prob & 0.2\\
\hline
node\_delete\_prob & 0.2\\
\hline
num\_hidden & 0\\
\hline
num\_inputs & N/A$^{\mathrm{a}}$\\
\hline
num\_outputs & N/A$^{\mathrm{a}}$\\
\hline
response\_init\_mean & 1.0\\
\hline
response\_init\_stdev & 0.0\\
\hline
response\_init\_type & gaussian\\
\hline
response\_max\_value & 30.0\\
\hline
response\_min\_value & -30.0\\
\hline
response\_mutate\_power & 0.0\\
\hline
response\_mutate\_rate & 0.0\\
\hline
response\_replace\_rate & 0.0\\
\hline
weight\_init\_mean & 0.0\\
\hline
weight\_init\_stdev & 1.0\\
\hline
weight\_init\_type & gaussian\\
\hline
weight\_max\_value & 30\\
\hline
weight\_min\_value & -30\\
\hline
weight\_mutate\_power & 0.5\\
\hline
weight\_mutate\_rate & 0.8\\
\hline
weight\_replace\_rate & 0.1\\
\hline
\multicolumn{2}{l}{$^{\mathrm{a}}$: Dependant on the experiment.}
\end{tabular}
\label{neat_table}
\end{center}
\end{table}


==> misc/NEAT_table_description.tex <==

\begin{table}[htbp]
\caption{NEAT Parameter Selection}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline\multicolumn{3}{|c|}{\textbf{Evolutionary Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}& \textbf{\textit{Description}}\\
\hline
pop\_size & 300 & Size of population \\
\hline
reset\_on\_extinction & False & Reset training if extinct\\
\hline
no\_fitness\_termination & True & Ignore early termination\\
\hline
\multicolumn{3}{|c|}{\textbf{Stagnation Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}& \textbf{\textit{Description}}\\
\hline
species\_fitness\_func & mean & To evaluate species fitness\\
\hline
max\_stagnation & 20 & Causes species extinction \\
\hline
species\_elitism & 2 & Elite species protected \\
\hline
\multicolumn{3}{|c|}{\textbf{Reproduction Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}& \textbf{\textit{Description}}\\
\hline
elitism & 2 & Elite members protected \\
\hline
survival\_threshold & 0.2 & Members able to reproduce\\
\hline
min\_species\_size & 2 & Minimum species size \\
\hline
\multicolumn{3}{|c|}{\textbf{Species Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}& \textbf{\textit{Description}}\\
\hline
compatibility\_threshold & 3.0 & Species differentiation \\
\hline
\multicolumn{3}{|c|}{\textbf{Genome Parameters}} \\
\hline
\textbf{\textit{Parameter}}& \textbf{\textit{Value}}& \textbf{\textit{Description}}\\
\hline
activation\_default & sigmoid & Default network activation \\
\hline
activation\_mutate\_rate & 0.0 & Mutation rate of activation\\
\hline
activation\_options & sigmoid & Options for activations\\
\hline
aggregation\_default & sum & Default network aggregation\\
\hline
aggregation\_mutate\_rate & 0.0 & Mutation rate of aggregation \\
\hline
aggregation\_options & sum & Options for aggregation \\
\hline
bias\_init\_mean & 0.0 & Initial node bias mean\\
\hline
bias\_init\_stdev & 1.0 & Initial node bias stdev\\
\hline
bias\_init\_type & gaussian & Bias initialization type \\
\hline
bias\_max\_value & 30.0 & Bias max value \\
\hline
bias\_min\_value & -30.0 & Bias min value \\
\hline
bias\_mutate\_power & 0.5 & Bias mutation stdev \\
\hline
bias\_mutate\_rate & 0.7 & Rate of bias mutation \\
\hline
bias\_replace\_rate & 0.1 & Rate of replacing bias\\
\hline
compatibility\_disjoint\_coefficient & 1.0 & Species differentiation \\
\hline
compatibility\_weight\_coefficient & 0.5 & Species differentiation \\
\hline
conn\_add\_prob & 0.5 & Rate of adding connection \\
\hline
conn\_delete\_prob & 0.5 & Rate of removing connection \\
\hline
enabled\_default & True & Whether genes start enabled \\
\hline
enabled\_mutate\_rate & 0.01 & Mutate rate for 'enabled'\\
\hline
feed\_forward & True & Network type \\
\hline
initial\_connection & full\_nodirect & Initial connection type \\
\hline
node\_add\_prob & 0.2 & Rate of adding nodes\\
\hline
node\_delete\_prob & 0.2 & Rate of removing nodes\\
\hline
num\_hidden & 0 & Initial hidden nodes \\
\hline
num\_inputs & N/A & Depends on problem\\
\hline
num\_outputs & N/A & Depends on problem\\
\hline
response\_init\_mean & 1.0 & Initial node response mean \\
\hline
response\_init\_stdev & 0.0 & Initial node response stdev\\
\hline
response\_init\_type & gaussian & Response initialization type\\
\hline
response\_max\_value & 30.0 & Response max value \\
\hline
response\_min\_value & -30.0 & Response min value\\
\hline
response\_mutate\_power & 0.0 & Response mutation stdev\\
\hline
response\_mutate\_rate & 0.0 & Response mutation rate\\
\hline
response\_replace\_rate & 0.0 & Response replacement rate \\
\hline
weight\_init\_mean & 0.0 & Initial weight mean \\
\hline
weight\_init\_stdev & 1.0 & Initial weight stdev \\
\hline
weight\_init\_type & gaussian & Weight initialization type\\
\hline
weight\_max\_value & 30 &  Weight max value\\
\hline
weight\_min\_value & -30 & Weight min value\\
\hline
weight\_mutate\_power & 0.5 & Weight mutation stdev \\
\hline
weight\_mutate\_rate & 0.8 & Weight mutation rate \\
\hline
weight\_replace\_rate & 0.1 & Weight replacement rate\\
\hline

\end{tabular}
\label{neat_table}
\end{center}
\end{table}


==> parts/acknow.tex <==
\section*{Acknowledgements}
\label{acknowledge}
DRAFT:
\begin{itemize}
    \item Not sure if necessary, since we would put these in references?
    \item GT for the blimps
    \item NRL for the lab space
\end{itemize}
